Real Time Vehicle Identification: A Synchronous-Transmission Based Approach

Identification of the vehicles passing over the roads is a very important component of traffic monitoring/surveillance. There have been many attempts to design and develop efficient strategies to carry out the job. However, from the point of view of practical usefulness and real-time operation, most of them do not score well. In the current work, we perceive the problem as efficient real-time communication and data-sharing between the units in charge of recording the identities of the vehicles, i.e., Vehicle Recorders (VR), and the Vehicles (VE). We propose a strategy to address the issue with the help of Synchronous-Transmission (ST), which is a newer paradigm of communication compared to the traditional paradigm based on Asynchronous-Transmission (AT). First, we theoretically show that the presence of the physical layer phenomena called Capture-Effect in ST brings a significant benefit. Next, we also implement the strategy in a well-known IoT-Operating System Contiki, and compare its performance with the existing best-known strategy.

==> 3-related.tex <==
\section{Related works}
\label{sec:related}



==> 5-simulation.tex <==
\section{Design}
\label{sec:design}


